Adversarial Pixel-Level Generation of Semantic Images

Generative Adversarial Networks (GANs) have obtained extraordinary success in the generation of realistic images, a domain where a lower pixel-level accuracy is acceptable. We study the problem, not yet tackled in the literature, of generating semantic images starting from a prior distribution. Intuitively this problem can be approached using standard methods and architectures. However, a better-suited approach is needed to avoid generating blurry, hallucinated and thus unusable images since tasks like semantic segmentation require pixel-level exactness. In this work, we present a novel architecture for learning to generate pixel-level accurate semantic images, namely Semantic Generative Adversarial Networks (SemGANs). The experimental evaluation shows that our architecture outperforms standard ones from both a quantitative and a qualitative point of view in many semantic image generation tasks.

==> pictures/facades/fid/show_fid.tex <==
\begin{figure*}[htb]

\bgroup 
 \def\arraystretch{0.2} 
 \setlength\tabcolsep{0.2pt}
\begin{tabular}{cc}
SeGAN \hspace{1cm}& GAN \\ 
\includegraphics[width=0.2\linewidth]{pictures/facades/fid/sgan_grid.png}  \hspace{1cm}&
\includegraphics[width=0.2\linewidth]{pictures/facades/fid/gan_grid.png} \\ 
\end{tabular} \egroup 

\vspace{-0.1in}
\caption{Comparison of the models yielding the best FID.}
\label{fig:facades-fid}
\end{figure*}

==> pictures/facades/show_facades.tex <==
\begin{figure*}[!htb]
\centering
\bgroup 
 \def\arraystretch{0.2} 
 \setlength\tabcolsep{0.2pt}
\begin{tabular}{cccc}
SeGAN \hspace{1cm}& GAN \hspace{5cm}& SeGAN \hspace{1cm}& GAN \\ 
\includegraphics[width=0.25\linewidth]{pictures/facades/swd/sgan_grid.png}  \hspace{1cm}&
\includegraphics[width=0.25\linewidth]{pictures/facades/swd/gan_grid.png}  \hspace{5cm}&
\includegraphics[width=0.25\linewidth]{pictures/facades/fid/sgan_grid.png}  \hspace{1cm}&
\includegraphics[width=0.25\linewidth]{pictures/facades/fid/gan_grid.png} \\
\end{tabular} \egroup 

\vspace{-0.1in}
\caption{Visual comparison for the facades experiment. Two figures on the left: models yielding the best average SWD. Two figures on the right: models yielding the best FID.}
\label{fig:facades}
\end{figure*}

==> pictures/facades/swd/show_swd.tex <==
\begin{figure*}[!htb]
\bgroup 
 \def\arraystretch{0.2} 
 \setlength\tabcolsep{0.2pt}
\begin{tabular}{cc}
SeGAN \hspace{1cm}& GAN \\ 
\includegraphics[width=0.2\linewidth]{pictures/facades/swd/sgan_grid.png}  \hspace{1cm}&
\includegraphics[width=0.2\linewidth]{pictures/facades/swd/gan_grid.png} \\ 
\end{tabular} \egroup 

\vspace{-0.1in}
\caption{Comparison of the models yielding the best average SWD.}
\label{fig:facades-swd}
\end{figure*}
